Modular Analysis of Tree-Topology Models

We investigate networks of automata that synchronise over common action labels. A graph synchronisation topology between the automata is defined in such a way that two automata are connected iff they can synchronise over an action. We show a very effective reduction of networks of automata with tree-like synchronisation topologies. The reduction preserves a certain form of reachability, but not safety. The procedure is implemented in an open-source tool.

==> experiments.tex <==
% !TEX root=./liveTrees.tex


==> live-reset.tex <==
% !TEX root=./liveTrees.tex

